Federated Causal Representation Learning in State-Space Systems for Decentralized Counterfactual Reasoning

Networks of interdependent industrial assets (clients) are tightly coupled through physical processes and control inputs, raising a key question: how would the output of one client change if another client were operated differently? This is difficult to answer because client-specific data are high-dimensional and private, making centralization of raw data infeasible. Each client also maintains proprietary local models that cannot be modified. We propose a federated framework for causal representation learning in state-space systems that captures interdependencies among clients under these constraints. Each client maps high-dimensional observations into low-dimensional latent states that disentangle intrinsic dynamics from control-driven influences. A central server estimates the global state-transition and control structure. This enables decentralized counterfactual reasoning where clients predict how outputs would change under alternative control inputs at others while only exchanging compact latent states. We prove convergence to a centralized oracle and provide privacy guarantees. Our experiments demonstrate scalability, and accurate cross-client counterfactual inference on synthetic and real-world industrial control system datasets.

==> ProblemFormulation.tex <==
We consider a system with $M$ clients. Each client $m \in \{1,\dots,M\}$ observes \textbf{high-dimensional measurements} $y_m^t \in \mathbb{R}^{D_m}$. Clients are equipped with proprietary models (fixed and non-modifiable) that output a \textbf{low-dimensional state estimate} $\hat{h}^t_{m,c} \in \mathbb{R}^{P_m}$ from local measurements $y_m^t$, with $D_m \gg P_m$. These proprietary models suffer from two limitations:  
\textbf{(1)} $\hat{h}^t_{m,c}$ encodes only local information and does not incorporate measurements from other clients (since they are trained solely on $y_m^t$).  
\textbf{(2)} $\hat{h}^t_{m,c}$ ignores external inputs from other clients, i.e., $u_n^t$ for all $n \neq m$.  As a result, proprietary models cannot answer counterfactual query \textbf{Q1}. To overcome these limitations, we adopt a federated learning framework involving all $M$ clients and a central server: 

\textbullet{} \textbf{(I) Client.} At each client $m$, the proprietary model is \textbf{augmented} with learnable parameters $\theta_m, \phi_m$ that \textit{implicitly} capture (i) the influence of other clients’ measurements and (ii) the effect of external inputs applied at other clients. The augmented client model outputs a state estimate $\hat{h}^t_{m,a}$, which incorporates both the proprietary estimate $\hat{h}^t_{m,c}$ and the corrections induced by $\theta_m, \phi_m$. Each client communicates $\hat{h}^t_{m,a}$, $\hat{h}^t_{m,c}$, and input $u_m^t$ to the server.

\textbullet{} \textbf{(II) Server.} The server aggregates information from all $M$ clients and explicitly estimates the cross-client parameters $\{A_{mn}, B_{mn}\}_{n \neq m}$. This is enforced via the server loss $L_s$, which encodes the estimated matrices. The server communicates only the gradients $\{\nabla_{h^t_{m,a}} L_s\}$ and $\{\nabla_{\hat{h}^{t-1}_{m,a}} L_s\}$ back to client $m$.

This design preserves privacy: \textit{client-to-server} communication ensures that raw measurements $y_m^t$ are never exposed beyond the client, while \textit{server-to-client} communication ensures that neither states $h_n^t$ nor inputs $u_n^t$ from other clients ($n \neq m$) are directly revealed. Thus, data-sharing and privacy constraints of the decentralized setting (Section~\ref{Sec:Counterfactual_Decentralized}) are respected.  

